An Experiment Combining Specialization with Abstract Interpretation

It was previously shown that control-flow refinement can be achieved by a program specializer incorporating property-based abstraction, to improve termination and complexity analysis tools. We now show that this purpose-built specializer can be reconstructed in a more modular way, and that the previous results can be achieved using an off-the-shelf partial evaluation tool, applied to an abstract interpreter. The key feature of the abstract interpreter is the abstract domain, which is the product of the property-based abstract domain with the concrete domain. This language-independent framework provides a practical approach to implementing a variety of powerful specializers, and contributes to a stream of research on using interpreters and specialization to achieve program transformations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{155}
\providecommand{\publicationstatus}{L. Fribourg and M. Heizmann (Eds.): VPT/HCVS 2020\\
EPTCS 320, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.320.11}{10.4204/EPTCS.320.11}}

